EvoDriveVLA: Evolving Driving VLA Models via Collaborative Perception-Planning Distillation

Vision-Language-Action models have shown great promise for autonomous driving, yet they suffer from degraded perception after unfreezing the visual encoder and struggle with accumulated instability in long-term planning. To address these challenges, we propose EvoDriveVLA-a novel collaborative perception-planning distillation framework that integrates self-anchored perceptual constraints and future-informed trajectory optimization. Specifically, self-anchored visual distillation leverages self-anchor teacher to deliver visual anchoring constraints, regularizing student representations via trajectory-guided key-region awareness. In parallel, future-informed trajectory distillation employs a future-aware oracle teacher with coarse-to-fine trajectory refinement and Monte Carlo dropout sampling to synthesize reasoning trajectories that model future evolutions, enabling the student model to internalize the future-aware insights of the teacher. EvoDriveVLA achieves SOTA performance in nuScenes open-loop evaluation and significantly enhances performance in NAVSIM closed-loop evaluation. Our code is available at: https://github.com/hey-cjj/EvoDriveVLA.

==> tables/Com_FSDrive.tex <==
\begin{table*}[t]
  \centering
  \caption{Compare with FSDrive using open-loop metrics.}
  \label{tab:ComFSD-open}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l cccc cccc | cccc cccc}
    \toprule
    \multirow{3}{*}{Method} & \multicolumn{8}{c}{ST-P3} & \multicolumn{8}{c}{UniAD} \\ 
    \cmidrule(lr){2-9} \cmidrule(lr){10-17}
    & \multicolumn{4}{c}{L2 (m) $\downarrow$} & \multicolumn{4}{c}{Collision (\%) $\downarrow$} & \multicolumn{4}{c}{L2 (m) $\downarrow$} & \multicolumn{4}{c}{Collision (\%) $\downarrow$} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
    
    FSDrive \footnotesize{[NIPS 25]} & 0.14 & 0.25 & 0.46 & 0.28 & 0.03 & 0.06 & 0.21 & 0.10 & 0.18 & 0.39 & \textbf{0.77} & \textbf{0.45} & \textbf{0.00} & 0.06 & 0.42 & 0.16 \\

    EvoDriveVLA(Ours) & \textbf{0.12} & \textbf{0.24} & \textbf{0.43} & \textbf{0.26} & \textbf{0.02} & \textbf{0.05} & \textbf{0.12} & \textbf{0.06} & \textbf{0.16} & 0.44 & 0.96 & 0.52 & 0.02 & \textbf{0.02} & \textbf{0.33} & \textbf{0.12} \\
    
    \bottomrule
    \end{tabular}
  }
  \vspace{0mm}
\end{table*}


\begin{table*}[t!]
    \centering
    \small
    \caption{\textbf{Compare with FSDrive using closed-loop metrics.}}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|cc|ccc|cc}
        \toprule
        Method & NC$\uparrow$ & DAC$\uparrow$ & TTC$\uparrow$ & Comf. $\uparrow$ & EP$\uparrow$ & PDMS$\uparrow$ \\
        \midrule
        
        FSDrive & \textbf{98.2} & \textbf{93.8} & \textbf{93.3} & 99.9 & 80.1 & \cellcolor{gray!30} 85.1 \\

        EvoDriveVLA(Ours) & 98.0 & 93.3 & 93.1 & \textbf{100} & \textbf{81.1} & \cellcolor{gray!30} \textbf{85.3} \\
        \bottomrule
    \end{tabular}
    \label{tab:ComFSD-closed}
\end{table*}
